Hyperbolic Fracton Model, Subsystem Symmetry and Holography III: Extension to Generic Tessellations

We generalize the Hyperbolic Fracton Model from the $\{5,4\}$ tessellation to generic tessellations, and investigate its core properties: subsystem symmetries, fracton mobility, and holographic correspondence. While the model on the original tessellation has features reminiscent of the flat-space lattice cases, the generalized tessellations exhibit a far richer and more intricate structure. The ground-state degeneracy and subsystem symmetries are generated recursively layer-by-layer, through the inflation rule, but without a simple, uniform pattern. The fracton excitations follow exponential-in-distance and algebraic-in-lattice-size growing patterns when moving outward, and depend sensitively to the tessellation geometry, differing qualitatively from both type-I or type-II fracton model on flat lattices. Despite this increased complexity, the hallmark holographic features -- subregion duality via Rindler reconstruction, the Ryu-Takayanagi formula for mutual information, and effective black hole entropy scaling with horizon area -- remain valid. These results demonstrate that the holographic correspondence in fracton models persists in generic tessellations, and provide a natural platform to explore more intricate subsystem symmetries and fracton physics.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{setspace}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}

\usepackage{color}  
\usepackage[colorlinks,linktocpage,bookmarks=false]{hyperref} 


\usepackage{graphicx}
\usepackage[left=20mm,right=20mm,top=30mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{float}
\usepackage{balance}              
\usepackage{tikz}                   
\usepackage{algpseudocode}
\usepackage{titling}
\usepackage{algorithm}
\usepackage{booktabs}
\usepackage{array} 
\usepackage{mdframed}
\usepackage{url}
\usepackage{libertine}
\usepackage{gensymb}
\usepackage{framed}
\usepackage{soul}
\usepackage{breqn}

\bibliographystyle{apsrev4-2}


\setlength{\parindent}{0cm}
\setlength{\parskip}{1ex plus 0.5ex minus 0.2ex}
\newcommand{\hsp}{\hspace{20pt}}
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}

\newmdtheoremenv{thm}{Theorem}
\theoremstyle{definition}
\newtheorem{exmp}{Example}[section]

\newcommand{\hy}[1]{{\color{blue} #1}}


